InfoMAE: Pair-Efficient Cross-Modal Alignment for Multimodal Time-Series Sensing Signals

Standard multimodal self-supervised learning (SSL) algorithms regard cross-modal synchronization as implicit supervisory labels during pretraining, thus posing high requirements on the scale and quality of multimodal samples. These constraints significantly limit the performance of sensing intelligence in IoT applications, as the heterogeneity and the non-interpretability of time-series signals result in abundant unimodal data but scarce high-quality multimodal pairs. This paper proposes InfoMAE, a cross-modal alignment framework that tackles the challenge of multimodal pair efficiency under the SSL setting by facilitating efficient cross-modal alignment of pretrained unimodal representations. InfoMAE achieves \textit{efficient cross-modal alignment} with \textit{limited data pairs} through a novel information theory-inspired formulation that simultaneously addresses distribution-level and instance-level alignment. Extensive experiments on two real-world IoT applications are performed to evaluate InfoMAE's pairing efficiency to bridge pretrained unimodal models into a cohesive joint multimodal model. InfoMAE enhances downstream multimodal tasks by over 60% with significantly improved multimodal pairing efficiency. It also improves unimodal task accuracy by an average of 22%.

==> figure/call/domain_generalization.tex <==
% \begin{figure}[t!]
% \centering
% \includegraphics[width=0.8\textwidth]{figure/sources/domain_generalization.pdf}
% \caption{Performance on Domain Generalization.}
% \label{fig:domain_generalization}
% \end{figure} 

\begin{figure}[!t]
\centering
\includegraphics[width=0.50\textwidth]{figure/sources/domain_generalization.pdf}
\caption{Performance on Domain Generalization.}
\label{fig:domain_generalization}
\end{figure}

==> figure/call/sparse_accuracy.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=0.47\textwidth]{figure/sources/sparse_accuracy.pdf}
\vspace{-0.4cm}
\caption{Cross-modal alignment with limited multimodal pairs.}
\label{fig:unimodal}
\end{figure}



==> figure/call/tsne_mod.tex <==
\begin{figure*}[t!]
  \centering
  \subfigure[InfoMAE]{\includegraphics[width=0.245\textwidth]{figure/sources/tsne_all/sample_MOD_SW-T_InfoMAE_use_proj.pdf}\label{fig:tsne_infomae}}
  \subfigure[FOCAL]{\includegraphics[width=0.245\textwidth]{figure/sources/tsne_all/sample_MOD_SW-T_FOCAL_use_proj.pdf}\label{fig:tsne_focal}}
  \subfigure[CMC]{\includegraphics[width=0.245\textwidth]{figure/sources/tsne_all/sample_MOD_SW-T_CMC.pdf}\label{fig:tsne_cmc}}
  \subfigure[GMC]{\includegraphics[width=0.245\textwidth]{figure/sources/tsne_all/sample_MOD_SW-T_GMC.pdf}\label{fig:tsne_gmc}}
  \label{fig:tsne_compare_deepsense}
  \caption{t-SNE visualization on MOD dataset}
%  \vspace{-0.3cm}
\end{figure*}

==> text/equations/cid.tex <==
% \begin{equation}
%     \begin{aligned}
%         \text{minimize} &\quad I(X_1, U_1) + I(X_2, U_2)\\
%         \text{s.t.} &\quad X_1 \condind X_2 \mid U_1 \\
%         &\quad X_1 \condind X_2 \mid U_2 \\
%         &\quad U_1 = U_2
%     \end{aligned}
% \end{equation}
% \begin{definition}
%     (Common Representation). Given a multimodal input $\mathcal{X}$, there exists a common representation $\mathcal{U}$ that can solve any task that requires common information in
% \end{definition}
\begin{equation}
    \begin{aligned}[c]
        \text{minimize} &\quad H(\mathcal{U})\\
        \text{s.t.}
        % &\quad X_1 \condind X_2 \mid U_1 \\
        % &\quad X_1 \condind X_2 \mid U_2 \\
        &\quad X_1 \condind X_2 \mid \mathcal{U} \\
        &\quad U_1 = U_2
    \end{aligned}
    \qquad\Longrightarrow\qquad
    \begin{aligned}[c]
        \text{minimize} &\quad I(X_1, U_1) + I(X_2, U_2)\\
        \text{s.t.} &\quad X_1 \condind X_2 \mid U_1 \\
        &\quad X_1 \condind X_2 \mid U_2 \\
        &\quad U_1 = U_2,
    \end{aligned}
\end{equation}
% \begin{definition}
%     (Common Representation). Given a multimodal input $\mathcal{X}$, there exists a common representation $\mathcal{U}$ that can solve any task that requires common information in
% \end{definition}

==> text/equations/cid2.tex <==
% \begin{equation}\label{equation:common_objective}
    
% \end{equation}

\begin{align*}
\text{minimize} &\ \ \ \sum_{i \in M} I(X_i, U_i) \\
\text{s.t.} &\ \ \ X_1 \condind X_2 \condind \dots \condind X_M \mid U_i \\
&\ \ \ U_i = U_j \mid \forall i, j \in M.
\end{align*}

==> text/equations/shared_loss_2.tex <==
\begin{equation}\label{shared_final}
    \mathcal{L}_\text{common} = \sum_{i \in M}\left( I(X_1; X_2; \dots X_M | U_{i}) + \beta I(X_{i}, U_{i})\right) + \sum_{i \in M}\sum_{j \neq i \in M}\alpha d(U_i - U_j)
\end{equation}

==> text/tables/KNN_evaluation_short.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[tp]
\caption{KNN Evaluation Results with SW-T encoder.}
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}c|cc|cc|cc|cc@{}}
\toprule
  \multirow{2}{*}{Framework} &
  \multicolumn{2}{c|}{MOD} &
  \multicolumn{2}{c|}{ACIDS} &
  \multicolumn{2}{c|}{RealWorld-HAR} &
  \multicolumn{2}{c}{PAMAP2} \\
                            & Acc    & F1     & Acc    & F1     & Acc             & F1              & Acc    & F1     \\ \midrule
SimCLR & 0.9022 & 0.9021 & 0.8553 & 0.7086 & 0.6532          & 0.6767          & 0.7441 & 0.7178 \\
                            MoCo   & 0.9344 & 0.9343 & 0.8311 & 0.6943 & 0.7103          & 0.7303          & 0.7082 & 0.6678 \\
                            CMC    & 0.8305 & 0.8261 & 0.7187 & 0.6355 & 0.5701          & 0.6007          & 0.7709 & 0.7694 \\
                            MAE    & 0.3389 & 0.3104 & 0.5945 & 0.4194 & 0.6428          & 0.6080          & 0.5517 & 0.4969 \\
                            Cosmo  & 0.2786 & 0.2621 & 0.5790 & 0.4573 & 0.7086          & 0.6389          & 0.6672 & 0.5874 \\
                            Cocoa  & 0.5941 & 0.5793 & 0.5311 & 0.4261 & 0.7421          & 0.7496          & 0.7188 & 0.7070 \\
                            MTSS   & 0.3423 & 0.3376 & 0.3151 & 0.1890 & 0.4882          & 0.4431          & 0.2007 & 0.1649 \\
                            TS2Vec & 0.5847 & 0.5718 & 0.6050 & 0.4144 & 0.5580          & 0.5335          & 0.5623 & 0.5040 \\
                            GMC    & 0.5318 & 0.5180 & 0.7589 & 0.6150 & 0.7380          & 0.7455          & 0.7567 & 0.7401 \\
                            TNC    & 0.8265 & 0.8263 & 0.7795 & 0.6725 & 0.8009          & 0.7817          & 0.7674 & 0.7189 \\
                            TSTCC  & 0.8607 & 0.8613 & 0.8356 & 0.6700 & 0.7582          & 0.7512          & 0.7780 & 0.7369 \\ \midrule
  \textbf{FOCAL} &
  \textbf{0.9665} &
  \textbf{0.9664} &
  \textbf{0.8826} &
  \textbf{0.7643} &
  \textbf{0.8586} &
  \textbf{0.8665} &
  \textbf{0.8549} &
  \textbf{0.8484} \\ \bottomrule
\end{tabular}%
}
\label{table:knn}
\end{table}

==> text/tables/additional_downstream.tex <==
\begin{table*}[t!]
\centering
\caption{Performance on additional tasks within the MOD dataset.}
% \yatong{Do SimCLR and MoCo get the same results? -> Yes}
\label{tab:additional_task}
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{@{}cc|cccc@{}}
\toprule
\multicolumn{2}{c|}{Dataset}                           & \multicolumn{4}{c}{MOD}                                                                                \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{Encoder}} & \multirow{2}{*}{Frameworks} & \multicolumn{2}{c|}{Distance Classification} & \multicolumn{2}{c}{Speed Classification} \\
\multicolumn{1}{c|}{}                       &          & Acc             & \multicolumn{1}{c|}{F1}              & Acc                   & F1                    \\ \midrule
\multicolumn{1}{c|}{\multirow{11}{*}{SW-T}} & SimCLR   & 0.9090          & \multicolumn{1}{c|}{0.8694}          & 0.5511                & 0.5514                \\
\multicolumn{1}{c|}{}                       & MoCo     & 0.9090          & \multicolumn{1}{c|}{0.8694}          & 0.6108                & {\ul \textit{0.6105}} \\ \cmidrule(l){2-6} 
\multicolumn{1}{c|}{}                       & CMC      & 0.8180          & \multicolumn{1}{c|}{0.7507}          & 0.5170                & 0.5175                \\
\multicolumn{1}{c|}{}                       & GMC      & 0.8181          & \multicolumn{1}{c|}{0.7450}          & 0.4460                & 0.4405                \\
\multicolumn{1}{c|}{}                       & FOCAL    & \textbf{0.9849} & \multicolumn{1}{c|}{\textbf{0.9726}} & \textbf{0.8329}       & \textbf{0.6920}       \\ \cmidrule(l){2-6} 
\multicolumn{1}{c|}{}                       & TNC      & 0.8484          & \multicolumn{1}{c|}{0.8015}          & 0.4375                & 0.4322                \\
\multicolumn{1}{c|}{}                       & TS-TCC   & 0.7878          & \multicolumn{1}{c|}{0.6575}          & 0.5284                & 0.5230                \\ \cmidrule(l){2-6} 
\multicolumn{1}{c|}{}                       & MMAE     & 0.7272          & \multicolumn{1}{c|}{0.4917}          & 0.4545                & 0.4383                \\
\multicolumn{1}{c|}{}                       & CAV-MAE  & 0.XXX     & \multicolumn{1}{c|}{0.XXX}     & 0.XXX           & 0.XXX           \\
\multicolumn{1}{c|}{}                       & MultiMAE & 0.XXX     & \multicolumn{1}{c|}{0.XXX}     & 0.XXX           & 0.XXX           \\ \cmidrule(l){2-6} 
\multicolumn{1}{c|}{}                       & InfoMAE  & \textbf{0.9849} & \multicolumn{1}{c|}{\textbf{0.9726}} & {\ul \textit{0.8002}} & 0.6056                \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> text/tables/datasets.tex <==
\begin{table}[!t]
\centering
\caption{Cross-modal Alignment Dataset. Domains used for supervised evaluation are bolded.}
\label{tab:alignment_domain}
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{@{}c|c|c@{}}
\toprule
Application &
  Modalities &
  Domains \\ \midrule
\begin{tabular}[c]{@{}c@{}}Moving Object\\ Detection (MOD)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}seismic\\ acoustic\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}domain M\\ domain G\\ domain T\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}Human Activity\\ Recognition (HAR)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}accelerometer\\ gyroscope\\ magnetometer\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PAMAP2\\ RealWorld-HAR\end{tabular} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> text/tables/domain_generalization.tex <==
\begin{table}[]
\centering
\caption{Performance of Joint Pretraining on MOD (seismic and acoustic) dataset and then finetuned on unseen domains.}
\label{tab:domain_generalization}
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{@{}cl|cc|cc@{}}
\toprule
\multicolumn{2}{c|}{Domain}  & \multicolumn{2}{c|}{\textbf{Domain G}} & \multicolumn{2}{c}{\textbf{Domain T}} \\ \midrule
\multicolumn{2}{c|}{Frameworks} & Acc    & F1     & Acc    & F1     \\ \midrule
\multicolumn{2}{c|}{CMC~\cite{chen2021mocov3}}        & 0.7924 & 0.7897 & 0.6791 & 0.6776 \\
\multicolumn{2}{c|}{FOCAL~\cite{liu2024focal}}      & 0.9137 & 0.9111 & 0.8156 & 0.8130 \\
\multicolumn{2}{c|}{GMC~\cite{poklukar2022gmc}}        & 0.7986 & 0.7947 & 0.3457 & 0.3387 \\
\multicolumn{2}{c|}{MoCo~\cite{chen2021mocov3}}       & 0.8719 & 0.8688 & 0.7500 & 0.7483 \\
\multicolumn{2}{c|}{SimCLR~\cite{chen2020simclr}}     & 0.8418 & 0.8386 & 0.7288 & 0.7207 \\
\multicolumn{2}{c|}{TNC~\cite{tonekaboni2021unsupervised}}        & 0.6916 & 0.6797 & 0.5680 & 0.5625 \\
\multicolumn{2}{c|}{TSTCC~\cite{eldele2021time}}      & 0.7080 & 0.7004 & 0.5804 & 0.5766 \\
\multicolumn{2}{c|}{MAE~\cite{he2022mae}}        & 0.6708 & 0.6642 & 0.4421 & 0.4365 \\
\multicolumn{2}{c|}{CAV-MAE~\cite{gong2022contrastive}}    & 0.5507 & 0.5282 & 0.3457 & 0.3387 \\\cmidrule(r){1-6}
\multicolumn{2}{c|}{\textbf{InfoMAE}} & \textbf{0.9196}    & \textbf{0.9186}   & \textbf{0.8546}   & \textbf{0.8535}   \\ \bottomrule
\end{tabular}%
}
\end{table}

==> text/tables/domain_shift.tex <==
\begin{table*}[t!]
\centering
\caption{Performance on Domain Generalization}
\label{tab:domain_shift}
\resizebox{0.80 \textwidth}{!}{%
\begin{tabular}{@{}cc|cc|cc|cc@{}}
\toprule
\multicolumn{2}{c|}{Datasets} &
  \multicolumn{2}{c|}{MOD} &
  \multicolumn{2}{c|}{Domain G} &
  \multicolumn{2}{c}{Domain T} \\ \midrule
\multicolumn{1}{c|}{Encoder} & Frameworks & Acc    & F1     & Acc    & F1     & Acc    & F1     \\ \midrule
\multicolumn{1}{c|}{\multirow{10}{*}{SW-T}} &
  SimCLR &
  0.9250 &
  0.9247 &
  0.8418 &
  0.8386 &
  0.7288 &
  0.7207 \\
\multicolumn{1}{c|}{}        & MoCo       & 0.9390 & 0.9384 & 0.8719 & 0.8688 & 0.7500 & 0.7483 \\ \cmidrule(l){2-8} 
\multicolumn{1}{c|}{}        & CMC        & 0.9129 & 0.9105 & 0.7924 & 0.7897 & 0.6791 & 0.6776 \\
\multicolumn{1}{c|}{}        & GMC        & 0.8640 & 0.8611 & 0.7986 & 0.7947 & 0.3457 & 0.3387 \\
\multicolumn{1}{c|}{} &
  FOCAL &
  {\ul \textit{0.9772}} &
  {\ul \textit{0.9765}} &
  {\ul \textit{0.9137}} &
  {\ul \textit{0.9111}} &
  {\ul \textit{0.8156}} &
  {\ul \textit{0.8130}} \\ \cmidrule(l){2-8} 
\multicolumn{1}{c|}{}        & TNC        & 0.8533 & 0.8539 & 0.6916 & 0.6797 & 0.5680 & 0.5625 \\
\multicolumn{1}{c|}{}        & TSTCC      & 0.8734 & 0.8735 & 0.7080 & 0.7004 & 0.5804 & 0.5766 \\ \cmidrule(l){2-8} 
\multicolumn{1}{c|}{}        & MAE        & 0.7803 & 0.7772 & 0.6708 & 0.6642 & 0.4421 & 0.4365 \\
\multicolumn{1}{c|}{}        & CAV-MAE    & 0.5821 & 0.5534 & 0.5507 & 0.5282 & 0.3457 & 0.3387 \\ \cmidrule(l){2-8} 
\multicolumn{1}{c|}{} &
  InfoMAE &
  \textbf{0.9826} &
  \textbf{0.9819} &
  \textbf{0.9196} &
  \textbf{0.9186} &
  \textbf{0.8546} &
  \textbf{0.8535} \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> text/tables/finetune.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\caption{Finetune Results with Linear Classifier}
\label{table:finetune}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}cc|cc|cc|cc|cc@{}}
\toprule
\multicolumn{2}{c|}{Dataset}                                  & \multicolumn{2}{c|}{MOD }          & \multicolumn{2}{c|}{ACIDS}        & \multicolumn{2}{c|}{RealWorld-HAR} & \multicolumn{2}{c}{PAMAP2}        \\ \midrule
\multicolumn{1}{c|}{Encoder}                     & Framework  & Acc             & F1              & Acc             & F1              & Acc              & F1              & Acc             & F1              \\ \midrule
\multicolumn{1}{c|}{\multirow{13}{*}{DeepSense}} & Supervised & 0.9404                & 0.9399                 & \textbf{0.9566}                 & 0.8407                 & 0.9348                  & \textbf{0.9388}                 & \textbf{0.8849}                 & \textbf{0.8761}                 \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{}                            & SimCLR     & 0.8855          & 0.8855          & 0.7438          & 0.6101          & 0.7138           & 0.6841          & 0.6802          & 0.6583          \\
\multicolumn{1}{c|}{}                            & MoCo       & 0.8808          & 0.8812          & 0.7717          & 0.6205          & 0.7859           & 0.7708          & 0.7559          & 0.7387          \\
\multicolumn{1}{c|}{}                            & CMC        & 0.9196          & 0.9186          & 0.8443          & 0.7244          & 0.7975           & 0.8116          & 0.7906          & 0.7706          \\
\multicolumn{1}{c|}{}                            & MAE        & 0.5981          & 0.5993          & 0.6644          & 0.5618          & 0.7565           & 0.7515          & 0.7114          & 0.6158          \\
\multicolumn{1}{c|}{}                            & Cosmo      & 0.8989          & 0.8998          & 0.8511          & 0.6929          & 0.8956           & 0.8888          & 0.8356          & 0.8135          \\
\multicolumn{1}{c|}{}                            & Cocoa      & 0.8774          & 0.8764          & 0.6644          & 0.5359          & 0.8465           & 0.8488          & 0.7603          & 0.7187          \\
\multicolumn{1}{c|}{}                            & MTSS       & 0.4153          & 0.3582          & 0.4352          & 0.2441          & 0.2989           & 0.1405          & 0.3541          & 0.1795          \\
\multicolumn{1}{c|}{}                            & TS2Vec     & 0.7669          & 0.7648          & 0.5224          & 0.3587          & 0.6595           & 0.5984          & 0.5729          & 0.4715          \\
\multicolumn{1}{c|}{}                            & GMC        & 0.9257          & 0.9267          & 0.9096          & 0.7929          & 0.8869           & 0.8948          & 0.8119          & 0.7860          \\
\multicolumn{1}{c|}{}                            & TNC        & 0.9518          & 0.9528          & 0.8237          & 0.6936          & 0.8892           & 0.8971          & 0.8387          & 0.8143          \\
\multicolumn{1}{c|}{}                            & TS-TCC     & 0.8707          & 0.8735          & 0.7667          & 0.6164          & 0.8073           & 0.8010          & 0.7776          & 0.7250          \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{}                            & \model     & \textbf{0.9732} & \textbf{0.9729} & 0.9516 & \textbf{0.8580} & \textbf{0.9382}  & 0.9290 & 0.8588 & 0.8463 \\ \midrule
\multicolumn{1}{c|}{\multirow{13}{*}{SW-T}}      & Supervised & 0.8948                & 0.8931                 & 0.9137                 & 0.7770                 & 0.9313                  & 0.9278                 & \textbf{0.8612}                 & 0.8384                 \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{}                            & SimCLR     & 0.9250          & 0.9247          & 0.9128          & 0.8144          & 0.7046           & 0.7220          & 0.7705          & 0.7424          \\
\multicolumn{1}{c|}{}                            & MoCo       & 0.9390          & 0.9384          & 0.9174          & 0.8100          & 0.7813           & 0.8024          & 0.7717          & 0.7313          \\
\multicolumn{1}{c|}{}                            & CMC        & 0.9129          & 0.9105          & 0.8128          & 0.6857          & 0.8840           & 0.8955          & 0.8080          & 0.7901          \\
\multicolumn{1}{c|}{}                            & MAE        & 0.7803          & 0.7772          & 0.8516          & 0.7023          & 0.8829           & 0.8813          & 0.7910          & 0.7606          \\
\multicolumn{1}{c|}{}                            & Cosmo      & 0.3429          & 0.3378          & 0.7110          & 0.6086          & 0.8604           & 0.8169          & 0.7741          & 0.7366          \\
\multicolumn{1}{c|}{}                            & Cocoa      & 0.7040          & 0.7038          & 0.7096          & 0.5794          & 0.8892           & 0.8861          & 0.7689          & 0.7317          \\
\multicolumn{1}{c|}{}                            & MTSS       & 0.4206          & 0.4163          & 0.3429          & 0.2250          & 0.5136           & 0.4370          & 0.2847          & 0.1714          \\
\multicolumn{1}{c|}{}                            & TS2Vec     & 0.7254          & 0.7174          & 0.7183          & 0.5748          & 0.6151           & 0.5955          & 0.6195          & 0.5426          \\
\multicolumn{1}{c|}{}                            & GMC        & 0.8640          & 0.8611          & 0.9402          & 0.7766          & 0.9319           & 0.9379          & 0.8312          & 0.8083          \\
\multicolumn{1}{c|}{}                            & TNC        & 0.8533          & 0.8539          & 0.8352          & 0.7372          & 0.8817           & 0.8784          & 0.8013          & 0.7506          \\
\multicolumn{1}{c|}{}                            & TS-TCC     & 0.8734          & 0.8735          & 0.9041          & 0.7547          & 0.8731           & 0.8454          & 0.7997          & 0.7260          \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{}                            & \model     & \textbf{0.9805} & \textbf{0.9800} & \textbf{0.9489} & \textbf{0.8262} & \textbf{0.9451}  & \textbf{0.9503} & 0.8580 & \textbf{0.8401} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> text/tables/finetune_results.tex <==
% \begin{table*}[]
% \centering
% \caption{Comparison with previous tasks on four datasets of two different tasks. The best and the second highest performance for SSL frameworks are marked by \textbf{bold} and \underline{\textit{underline}} respectively.}
% \label{tab:finetune}
% \resizebox{0.95 \textwidth}{!}{%
% \begin{tabular}{@{}cc|cccc|cccc@{}}
% \toprule
% \multicolumn{2}{c|}{Task} &
%   \multicolumn{4}{c|}{Vehicle Classification} &
%   \multicolumn{4}{c}{Activity Classification} \\ \midrule
% \multicolumn{2}{c|}{Datasets} &
%   \multicolumn{2}{c|}{MOD} &
%   \multicolumn{2}{c|}{ACIDS} &
%   \multicolumn{2}{c|}{RealWorld-HAR} &
%   \multicolumn{2}{c}{PAMAP2} \\ \midrule
% \multicolumn{1}{c|}{Encoder} &
%   Frameworks &
%   Acc &
%   \multicolumn{1}{c|}{F1} &
%   Acc &
%   F1 &
%   Acc &
%   \multicolumn{1}{c|}{F1} &
%   Acc &
%   F1 \\ \midrule
% \multicolumn{1}{c|}{\multirow{11}{*}{SW-T}} &
%   Supervised &
%   0.8948 &
%   \multicolumn{1}{c|}{0.8931} &
%   0.9137 &
%   0.7770 &
%   0.9313 &
%   \multicolumn{1}{c|}{0.9278} &
%   0.8612 &
%   0.8384 \\ \cmidrule(l){2-10} 
% \multicolumn{1}{c|}{} &
%   SimCLR &
%   0.9250 &
%   \multicolumn{1}{c|}{0.9247} &
%   0.9128 &
%   0.8144 &
%   0.7046 &
%   \multicolumn{1}{c|}{0.7220} &
%   0.7705 &
%   0.7424 \\
% \multicolumn{1}{c|}{} &
%   MoCo &
%   \textit{{\ul 0.9390}} &
%   \multicolumn{1}{c|}{\textit{{\ul 0.9384}}} &
%   0.9174 &
%   0.8100 &
%   0.7813 &
%   \multicolumn{1}{c|}{0.8024} &
%   0.7717 &
%   0.7313 \\ \cmidrule(l){2-10} 
% \multicolumn{1}{c|}{} &
%   CMC &
%   0.9129 &
%   \multicolumn{1}{c|}{0.9105} &
%   0.8128 &
%   0.6857 &
%   0.8840 &
%   \multicolumn{1}{c|}{0.8955} &
%   0.8080 &
%   0.7901 \\
% \multicolumn{1}{c|}{} &
%   GMC &
%   0.8640 &
%   \multicolumn{1}{c|}{0.8611} &
%   \textbf{0.9402} &
%   \textbf{0.7766} &
%   \textit{{\ul 0.9319}} &
%   \multicolumn{1}{c|}{\textit{{\ul 0.9379}}} &
%   \textit{{\ul 0.8312}} &
%   \textit{{\ul 0.8083}} \\ \cmidrule(l){2-10} 
% \multicolumn{1}{c|}{} &
%   TNC &
%   0.8533 &
%   \multicolumn{1}{c|}{0.8539} &
%   0.8352 &
%   0.7372 &
%   0.8817 &
%   \multicolumn{1}{c|}{0.8784} &
%   0.8013 &
%   0.7506 \\
% \multicolumn{1}{c|}{} &
%   TSTCC &
%   0.8734 &
%   \multicolumn{1}{c|}{0.8735} &
%   0.9041 &
%   0.7547 &
%   0.8731 &
%   \multicolumn{1}{c|}{0.8454} &
%   0.7997 &
%   0.7260 \\ \cmidrule(l){2-10} 
% \multicolumn{1}{c|}{} &
%   MMAE &
%   0.7803 &
%   \multicolumn{1}{c|}{0.7772} &
%   0.8516 &
%   0.7023 &
%   0.8829 &
%   \multicolumn{1}{c|}{0.8813} &
%   0.7910 &
%   0.7606 \\
% \multicolumn{1}{c|}{} &
%   CAV-MAE &
%   0.5184 &
%   \multicolumn{1}{c|}{0.4941} &
%   0.7995 &
%   0.6711 &
%   0.9215 &
%   \multicolumn{1}{c|}{0.9267} &
%   0.7697 &
%   0.7351 \\
% \multicolumn{1}{c|}{} &
%   MultiMAE &
%   0.XXX &
%   \multicolumn{1}{c|}{0.XXX} &
%   0.XXX &
%   0.XXX &
%   0.XXX &
%   \multicolumn{1}{c|}{0.XXX} &
%   0.XXX &
%   0.XXX \\ \cmidrule(l){2-10} 
% \multicolumn{1}{c|}{} &
%   InfoMAE &
%   \textbf{0.9826} &
%   \multicolumn{1}{c|}{\textbf{0.9819}} &
%   0.9101 &
%   0.7458 &
%   \textbf{0.9411} &
%   \multicolumn{1}{c|}{\textbf{0.9462}} &
%   \textbf{0.8478} &
%   \textbf{0.8319} \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

% % 0.9826  0.9819

\begin{table*}[t!]
\centering
\caption{Comparison with previous works on four datasets of two different tasks. The best and the second highest performance for SSL frameworks are marked by \textbf{bold} and \underline{\textit{underline}} respectively.}
\label{tab:finetune}
\resizebox{0.7 \textwidth}{!}{%
\begin{tabular}{@{}cc|cccc|cccc@{}}
\toprule
\multicolumn{2}{c|}{Task} &
  \multicolumn{4}{c|}{Vehicle Classification} &
  \multicolumn{4}{c}{Activity Classification} \\ \midrule
\multicolumn{2}{c|}{Datasets} &
  \multicolumn{2}{c|}{MOD} &
  \multicolumn{2}{c|}{ACIDS} &
  \multicolumn{2}{c|}{RealWorld-HAR} &
  \multicolumn{2}{c}{PAMAP2} \\ \midrule
\multicolumn{1}{c|}{Encoder} &
  Frameworks &
  Acc &
  \multicolumn{1}{c|}{F1} &
  Acc &
  F1 &
  Acc &
  \multicolumn{1}{c|}{F1} &
  Acc &
  F1 \\ \midrule
\multicolumn{1}{c|}{\multirow{11}{*}{SW-T}} &
  Supervised &
  0.8948 &
  \multicolumn{1}{c|}{0.8931} &
  0.9137 &
  0.7770 &
  0.9313 &
  \multicolumn{1}{c|}{0.9278} &
  0.8612 &
  0.8384 \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{} &
  SimCLR &
  0.9250 &
  \multicolumn{1}{c|}{0.9247} &
  0.9128 &
  {\ul \textit{0.8144}} &
  0.7046 &
  \multicolumn{1}{c|}{0.7220} &
  0.7705 &
  0.7424 \\
\multicolumn{1}{c|}{} &
  MoCo &
  0.9390 &
  \multicolumn{1}{c|}{0.9384} &
  0.9174 &
  0.8100 &
  0.7813 &
  \multicolumn{1}{c|}{0.8024} &
  0.7717 &
  0.7313 \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{} &
  CMC &
  0.9129 &
  \multicolumn{1}{c|}{0.9105} &
  0.8128 &
  0.6857 &
  0.8840 &
  \multicolumn{1}{c|}{0.8955} &
  0.8080 &
  0.7901 \\
\multicolumn{1}{c|}{} &
  GMC &
  0.8640 &
  \multicolumn{1}{c|}{0.8611} &
  {\ul \textit{0.9402}} &
  0.7766 &
  0.9319 &
  \multicolumn{1}{c|}{0.9379} &
  0.8312 &
  0.8083 \\
\multicolumn{1}{c|}{} &
  FOCAL &
  \multicolumn{1}{l}{{\ul \textit{0.9805}}} &
  \multicolumn{1}{l|}{{\ul \textit{0.9800}}} &
  \multicolumn{1}{l}{\textbf{0.9489}} &
  \multicolumn{1}{l|}{\textbf{0.8262}} &
  \multicolumn{1}{l}{\textbf{0.9451}} &
  \multicolumn{1}{l|}{\textbf{0.9503}} &
  \multicolumn{1}{l}{\textbf{0.8580}} &
  \textbf{0.8401} \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{} &
  TNC &
  0.8533 &
  \multicolumn{1}{c|}{0.8539} &
  0.8352 &
  0.7372 &
  0.8817 &
  \multicolumn{1}{c|}{0.8784} &
  0.8013 &
  0.7506 \\
\multicolumn{1}{c|}{} &
  TSTCC &
  0.8734 &
  \multicolumn{1}{c|}{0.8735} &
  0.9041 &
  0.7547 &
  0.8731 &
  \multicolumn{1}{c|}{0.8454} &
  0.7997 &
  0.7260 \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{} &
  MMAE &
  0.7803 &
  \multicolumn{1}{c|}{0.7772} &
  0.8516 &
  0.7023 &
  0.8829 &
  \multicolumn{1}{c|}{0.8813} &
  0.7910 &
  0.7606 \\
\multicolumn{1}{c|}{} &
  CAV-MAE &
  0.5821 &
  \multicolumn{1}{c|}{0.5534} &
  0.7995 &
  0.6711 &
  0.9215 &
  \multicolumn{1}{c|}{0.9267} &
  0.7697 &
  0.7351 \\ \cmidrule(l){2-10} 
\multicolumn{1}{c|}{} &
  InfoMAE &
  \textbf{0.9826} &
  \multicolumn{1}{c|}{\textbf{0.9819}} &
  0.9356 &
  0.8101 &
  {\ul \textit{0.9411}} &
  \multicolumn{1}{c|}{{\ul \textit{0.9462}}} &
  {\ul \textit{0.8478}} &
  {\ul \textit{0.8319}} \\ \bottomrule
\end{tabular}%
}
\end{table*}

% 0.9826  0.9819

==> text/tables/noaug.tex <==
\begin{table*}[t!]
\centering
\caption{Performance on additional tasks within the MOD dataset.}
\label{tab:additional_task}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}cc|cc@{}}
\toprule
\multicolumn{2}{c|}{Dataset}                            & \multicolumn{2}{c}{MOD}                  \\ \midrule
\multicolumn{1}{c|}{Encoder}               & Frameworks & \multicolumn{2}{c}{Acc}                       \\ \midrule
\multicolumn{1}{c|}{\multirow{8}{*}{SW-T}} & SimCLR     & 0.2143                & 0.1951                \\
\multicolumn{1}{c|}{}                      & MoCo       & 0.2391                & 0.2168                \\ \cmidrule(l){2-4} 
\multicolumn{1}{c|}{}                      & CMC        & 0.4153                & 0.4115                \\
\multicolumn{1}{c|}{}                      & GMC        & 0.2740                & 0.2421                \\
\multicolumn{1}{c|}{}                      & FOCAL      & {\ul \textit{0.8352}} & {\ul \textit{0.8325}} \\ \cmidrule(l){2-4} 
\multicolumn{1}{c|}{}                      & TNC        & 0.5285                & 0.5237                \\
\multicolumn{1}{c|}{}                      & TSTCC      & 0.4374                & 0.4194                \\ \cmidrule(l){2-4} 
\multicolumn{1}{c|}{}                      & InfoMAE    & \textbf{0.9337}       & \textbf{0.9333}       \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> text/tables/temp_to_baselines.tex <==
\begin{table}[t!]
\centering
\caption{Benefits of Temporal Constraints to SOTA baselines on ACIDS}
\label{tab:temporal_constraints_baselines_acids}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Metrics} &
  \multicolumn{2}{c|}{SimCLR} &
  \multicolumn{2}{c|}{MoCo} &
  \multicolumn{2}{c|}{CMC} &
  \multicolumn{2}{c|}{Cocoa} &
  \multicolumn{2}{c}{GMC} \\ \cmidrule(l){2-11} 
        & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 \\ \midrule
wTemp &
  \textbf{0.7461} &
  \textbf{0.6938} &
  \textbf{0.7836} &
  \textbf{0.6618} &
  \textbf{0.8690} &
  0.7090 &
  \textbf{0.8543} &
  \textbf{0.7665} &
  \textbf{0.9347} &
  \textbf{0.8109} \\
Vanilla & 0.7438       & 0.6101      & 0.7717       & 0.6205      & 0.8443       & \textbf{0.7244} & 0.6644       & 0.5359      & 0.9096       & 0.7929      \\ \bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[t!]
\centering
\caption{Benefits of Temporal Constraints to SOTA baselines on PAMAP2}
\label{tab:temporal_constraints_baselines_pamap2}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Metrics} &
  \multicolumn{2}{c|}{SimCLR} &
  \multicolumn{2}{c|}{MoCo} &
  \multicolumn{2}{c|}{CMC} &
  \multicolumn{2}{c|}{Cocoa} &
  \multicolumn{2}{c}{GMC} \\ \cmidrule(l){2-11} 
        & Acc    & F1     & Acc    & F1     & Acc             & F1              & Acc    & F1     & Acc    & F1     \\ \midrule
wTemp &
  \textbf{0.7129} &
  \textbf{0.6884} &
  \textbf{0.7800} &
  \textbf{0.7602} &
  0.7804 &
  0.7583 &
  \textbf{0.8442} &
  \textbf{0.8146} &
  \textbf{0.8253} &
  \textbf{0.8114} \\
Vanilla & 0.6802 & 0.6583 & 0.7559 & 0.7387 & \textbf{0.7906} & \textbf{0.7706} & 0.7603 & 0.7187 & 0.8119 & 0.7860 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> text/tables/unimodal.tex <==
% \begin{table}[]
% \centering
% \caption{Comparison on Unimodal Finetuning with and without InfoMAE Synchronization}
% \label{tab:my-table}
% \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{@{}c|cccccc@{}}
% \toprule
% \multirow{3}{*}{Modalities} & \multicolumn{6}{c}{MOD}                                                                              \\ \cmidrule(l){2-7} 
%                             & \multicolumn{2}{c|}{TP}              & \multicolumn{2}{c|}{GT}              & \multicolumn{2}{c}{TT} \\ \cmidrule(l){2-7} 
%                             & Acc    & \multicolumn{1}{c|}{F1}     & Acc    & \multicolumn{1}{c|}{F1}     & Acc        & F1        \\ \midrule
% Seismic w/o sync            & 0.2853 & \multicolumn{1}{c|}{0.2712} & 0.4273 & \multicolumn{1}{c|}{0.4119} & 0.3074     & 0.2977    \\
% Seismic with sync  & \textbf{0.3557} & \multicolumn{1}{c|}{\textbf{0.3339}} & \textbf{0.5271} & \multicolumn{1}{c|}{\textbf{0.5146}} & \textbf{0.3624} & \textbf{0.3408} \\ \midrule
% Acoustic w/o sync           & 0.6423 & \multicolumn{1}{c|}{0.6346} & 0.3416 & \multicolumn{1}{c|}{0.3333} & 0.3577     & 0.3520    \\
% Acoustic with sync & \textbf{0.7207} & \multicolumn{1}{c|}{\textbf{0.7088}} & \textbf{0.4561} & \multicolumn{1}{c|}{\textbf{0.4325}} & \textbf{0.4756} & \textbf{0.4345} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[]
\centering
\caption{Comparison on Unimodal Finetuning with and without InfoMAE Synchronization.}
\label{tab:my-table}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}c|cccccccccc@{}}
\toprule
\multirow{3}{*}{Modalities} &
  \multicolumn{10}{c}{MOD} \\ \cmidrule(l){2-11} 
 &
  \multicolumn{2}{c|}{TP} &
  \multicolumn{2}{c|}{GT} &
  \multicolumn{2}{c|}{TT} &
  \multicolumn{2}{c|}{GP} &
  \multicolumn{2}{c}{TG} \\ \cmidrule(l){2-11} 
 &
  Acc &
  \multicolumn{1}{c|}{F1} &
  Acc &
  \multicolumn{1}{c|}{F1} &
  Acc &
  \multicolumn{1}{c|}{F1} &
  Acc &
  \multicolumn{1}{c|}{F1} &
  Acc &
  F1 \\ \midrule
Seismic w/o sync &
  0.2853 &
  \multicolumn{1}{c|}{0.2712} &
  0.4273 &
  \multicolumn{1}{c|}{0.4119} &
  0.2853 &
  \multicolumn{1}{c|}{0.2712} &
  0.4273 &
  \multicolumn{1}{c|}{0.4119} &
  0.2853 &
  0.2712 \\
Seismic with sync &
  \textbf{0.3557} &
  \multicolumn{1}{c|}{\textbf{0.3339}} &
  \textbf{0.5271} &
  \multicolumn{1}{c|}{\textbf{0.5146}} &
  \textbf{0.3624} &
  \multicolumn{1}{c|}{\textbf{0.3408}} &
  \textbf{0.5177} &
  \multicolumn{1}{c|}{\textbf{0.4842}} &
  \textbf{0.3510} &
  \textbf{0.3201} \\ \midrule
Acoustic w/o sync &
  0.6423 &
  \multicolumn{1}{c|}{0.6346} &
  0.3416 &
  \multicolumn{1}{c|}{0.3333} &
  0.3416 &
  \multicolumn{1}{c|}{0.3333} &
  0.6423 &
  \multicolumn{1}{c|}{0.6346} &
  0.6410 &
  0.6332 \\
Acoustic with sync &
  \textbf{0.7207} &
  \multicolumn{1}{c|}{\textbf{0.7088}} &
  \textbf{0.4561} &
  \multicolumn{1}{c|}{\textbf{0.4325}} &
  \textbf{0.4756} &
  \multicolumn{1}{c|}{\textbf{0.4345}} &
  \textbf{0.7006} &
  \multicolumn{1}{c|}{\textbf{0.6829}} &
  \textbf{0.6999} &
  \textbf{0.6891} \\ \bottomrule
\end{tabular}%
}
\end{table}
